GeLLMO: Generalizing Large Language Models for Multi-property Molecule Optimization

Despite recent advancements, most computational methods for molecule optimization are constrained to single- or double-property optimization tasks and suffer from poor scalability and generalizability to novel optimization tasks. Meanwhile, Large Language Models (LLMs) demonstrate remarkable out-of-domain generalizability to novel tasks. To demonstrate LLMs' potential for molecule optimization, we introduce MuMOInstruct, the first high-quality instruction-tuning dataset specifically focused on complex multi-property molecule optimization tasks. Leveraging MuMOInstruct, we develop GeLLMOs, a series of instruction-tuned LLMs for molecule optimization. Extensive evaluations across 5 in-domain and 5 out-of-domain tasks demonstrate that GeLLMOs consistently outperform state-of-the-art baselines. GeLLMOs also exhibit outstanding zero-shot generalization to unseen tasks, significantly outperforming powerful closed-source LLMs. Such strong generalizability demonstrates the tremendous potential of GeLLMOs as foundational models for molecule optimization, thereby tackling novel optimization tasks without resource-intensive retraining. MuMOInstruct, models, and code are accessible through https://github.com/ninglab/GeLLMO.

==> figures/BHMQ_case.tex <==
\begin{figure}[t!]
    \centering
    \begin{minipage}{0.43\linewidth}
        \centering
        \tiny $M_x$
        \includegraphics[width=1.0\linewidth]{./figures/BHMQ_mollm_src.png}
        \par\vspace{2pt}
        \tiny BBBP=0.08, HIA=0.42, \\
        \tiny Mutag=0.60, QED=0.37
    \end{minipage}
    \hfill
    \begin{minipage}{0.05\linewidth}
        \centering
        \Large$\Rightarrow$\\
        \tiny \mollm
        %\raggedright\tiny \mollm
    \end{minipage}
    \hfill
    \begin{minipage}{0.43\linewidth}
        \centering
        \tiny $M_y$
        \includegraphics[width=1.0\linewidth]{./figures/BHMQ_mollm_opt.png}
        \par\vspace{2pt}
        \tiny BBBP=0.82 (+0.78), HIA=0.98 (+0.56),\\ 
        \tiny Mutag=0.30 (-0.30), QED=0.74 (+0.37)
    \end{minipage}
    \caption{{\mollmSixGenM} optimization example from \BHMQ. Modifications are highlighted in red.}
    \label{fig:case_BHMQ}

    \vspace{-15pt}
\end{figure}


==> tables/bdp_ind_old.tex <==
\begin{table*}[h!]
\centering
\caption{Overall Performance on \BDP}
\label{tbl:bdp_ind}
\begin{threeparttable}

\begin{tabular}{
    @{\hspace{3pt}}l@{\hspace{3pt}}
    @{\hspace{3pt}}l@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    @{\hspace{3pt}}r@{\hspace{3pt}}
    % @{\hspace{3pt}}r@{\hspace{3pt}}
    % @{\hspace{3pt}}r@{\hspace{3pt}}
}
\toprule
\multirow{2}{*}{Category} 
& \multirow{2}{*}{Model} 
& \multirow{2}{*}{\SR$^{\uparrow}$}
& \multirow{2}{*}{\Val$^{\uparrow}$} 
& \multirow{2}{*}{\Sim$^{\uparrow}$} 
& \multirow{2}{*}{\Nov$^{\uparrow}$}
& \multirow{2}{*}{\SAS$^{\downarrow}$}
& \multirow{2}{*}{\RI$^{\uparrow}$}
& \multicolumn{3}{c}{\APS}
%& \multicolumn{3}{c}{Property Improvement} 
\\
\cmidrule(lr){9-11} %\cmidrule(lr){10-12}
& & & & & & & & BBBP$\uparrow$ & DRD2$\uparrow$ & plogP$\uparrow$ 
%& bbbp$^{\uparrow}$ & drd2$^{\uparrow}$ & plogp$^{\uparrow}$
\\
\midrule
% \PMolTriple (TS) & 10.60 & 0.20 & 100.00 & 2.75 & 0.82 & 0.91 & 0.25 & 0.76 & 0.53 & 0.24 & 3.08 \\
% \PMolQuad (TS) & 7.20 & 0.13 & 100.00 & 2.61 & 0.84 & 0.93 & 0.19 & 0.64 & 0.55 & 0.18 & 3.06 \\
% \PMolTriple (G) & 73.00 & 0.45 & 99.18 & 2.91 & 0.86 & 0.82 & 0.21 & 0.57 & 0.48 & 0.21 & 2.77 \\
% \PMolQuad (G) & 77.00 & 0.47 & 99.74 & 2.98 & 0.86 & 0.80 & 0.22 & 0.69 & 0.45 & 0.21 & 2.84 \\

\multirow{6}{*}{General purpose LLMs}
 & Mistral (0-shot) & 6.60 & 75.00 & 0.81 & 100.00 & 3.72 & 0.47 & 0.03 & -0.91 \\
 & Llama (0-shot) & 22.00 & 85.60 & 0.73 & 100.00 & 3.95 & 0.58 & 0.03 & -1.94 \\
 & Claude-3.5 (0-shot) & 19.60 & 94.40 & 0.66 & 100.00 & 3.53 & 0.65 & 0.05 & -1.49 \\
 & Mistral (5-shot) & 35.20 & 95.20 & 0.64 & 96.59 & 3.42 & 0.66 & 0.11 & -0.87 \\
 & Llama (5-shot) & 35.40 & 96.80 & 0.57 & 79.10 & 3.50 & 0.64 & 0.17 & -0.83 \\
 & Claude-3.5 (5-shot) & 35.40 & 95.40 & 0.50 & 100.00 & 3.18 & 0.77 & 0.10 & -0.45 \\
\hline

Chemistry LLMs
& \LlaSMolM & 43.60 & 98.40 & 0.62 & 99.54 & 3.38 & 0.59 & 0.05 & -1.09 \\
\hline

Task-specific non-LLM 
& \PMol & 12.20 & 20.80 & 0.12 & 96.72 & 2.66 & 0.96 & 0.45 & 1.59 \\
\hline

\multirow{4}{*}{Task-specific LLMs}
%& \mollmTripleTaskM & 97.80 & 81.00 & 0.49 & 98.77 & 3.12 & 0.76 & 0.18 & 0.12 \\
& \mollmTripleTaskM & 84.80 & 96.80 & 0.47 & 100.00 & 3.06 & 0.77 & 0.23 & 0.46 \\
%& \mollmTripleTaskL & 99.00 & 84.00 & 0.50 & 98.33 & 2.86 & 0.75 & 0.24 & 0.40 \\
& \mollmTripleTaskL & 86.80 & 99.00 & 0.48 & 99.31 & 3.01 & 0.76 & 0.25 & 0.42 \\
& \mollmQuadTaskM & 50.40 & 97.60 & 0.63 & 100.00 & 3.13 & 0.65 & 0.09 & -0.62 \\
%& \mollmQuadTaskM & 97.60 & 50.40 & 0.63 & 100.00 & 3.13 & 0.65 & 0.09 & -0.62 \\
& \mollmQuadTaskL & 53.60 & 98.80 & 0.63 & 99.25 & 3.19 & 0.68 & 0.09 & -0.57 \\
\hline

\multirow{6}{*}{General purpose LLMs}
& \mollmTripleGenM & 75.60 & 98.20 & 0.56 & 100.00 & 3.18 & 0.68 & 0.16 & 0.07 \\
& \mollmTripleGenL & 77.40 & 99.00 & 0.51 & 99.74 & 3.10 & 0.74 & 0.16 & 0.04 \\

%& \mollmQuadGenM & 97.60 & 73.80 & 0.58 & 99.73 & 3.27 & 0.69 & 0.14 & -0.33 \\
%& \mollmQuadGenM & 97.60 & 76.20 & 0.58 & 99.74 & 3.24 & 0.68 & 0.14 & -0.10 \\
& \mollmQuadGenM  & 81.40 & 98.80 & 0.55 & 99.75 & 3.07 & 0.73 & 0.19 & 0.12 \\
& \mollmQuadGenL & 80.40 & 99.40 & 0.54 & 99.75 & 3.01 & 0.73 & 0.18 & 0.02 \\

& \mollmSixGenM & 83.00 & 98.80 & 0.57 & 99.76 & 3.17 & 3.60 & 0.72 & 0.17 & 0.12 \\
& \mollmSixGenL & 77.00 & 99.40 & 0.53 & 99.48 & 3.00 & 3.73 & 0.74 & 0.18 & 0.25 \\


\bottomrule
\end{tabular}





% \begin{tabular}{
%     @{\hspace{3pt}}l@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{10pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{10pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
%     @{\hspace{3pt}}r@{\hspace{3pt}}
% }
% \toprule
% \multirow{2}{*}{Model} 
% & \multirow{2}{*}{\SR$^{\uparrow}$} 
% & \multirow{2}{*}{\Sim$^{\uparrow}$} 
% & \multirow{2}{*}{\Nov$^{\uparrow}$}
% & \multirow{2}{*}{\SAS$^{\downarrow}$}
% & \multirow{2}{*}{\Div$^{\uparrow}$}
% & \multicolumn{3}{c}{Property Average}
% & \multicolumn{3}{c}{Property Improvement} 
% \\
% \cmidrule(lr){7-9} \cmidrule(lr){10-12}
% & & & & & & bbbp$^{\uparrow}$ & drd2$^{\uparrow}$ & plogp$^{\uparrow}$
% & bbbp$^{\uparrow}$ & drd2$^{\uparrow}$ & plogp$^{\uparrow}$
% \\
% \midrule
% % \PMolTriple (TS) & 0.00 & 0.00 \\
% % \PMolQuad (TS) & 0.00 & 0.00 \\
% % \PMolTriple (G) & 60.40 & 0.53 & 99.67 & 2.91 & 0.86 & 0.80 & 0.17 & 0.51 & 0.45 & 0.16 & 2.64 \\
% % \PMolQuad (G) & 65.00 & 0.54 & 100.00 & 2.94 & 0.85 & 0.78 & 0.20 & 0.71 & 0.43 & 0.19 & 2.66 \\
% \PMolTriple & 0.00 \\
% \hline
% Llama (0-shot) & 21.60 & 0.74 & 100.00 & 3.96 & 0.86 & 0.58 & 0.03 & -2.02 & 0.26 & 0.02 & 0.63 \\
% Mistral (0-shot) & 6.60 & 0.81 & 100.00 & 3.72 & 0.87 & 0.47 & 0.03 & -0.91 & 0.16 & 0.02 & 0.84 \\
% Claude-3.5 (0-shot) & 18.40 & 0.68 & 100.00 & 3.51 & 0.88 & 0.64 & 0.04 & -1.56 & 0.29 & 0.03 & 0.91 \\
% Llama (5-shot) & 28.60 & 0.72 & 100.00 & 3.74 & 0.88 & 0.58 & 0.05 & -1.70 & 0.25 & 0.04 & 0.85 \\
% Mistral (5-shot) & 33.20 & 0.68 & 100.00 & 3.45 & 0.88 & 0.65 & 0.08 & -1.04 & 0.30 & 0.07 & 0.99 \\
% Claude-3.5 (5-shot) & 25.00 & 0.60 & 100.00 & 3.31 & 0.87 & 0.71 & 0.06 & -1.17 & 0.37 & 0.05 & 1.68 \\

% \hline
% \LlaSMolM & 39.60 & 0.67 & 100.00 & 3.45 & 0.88 & 0.58 & 0.04 & -1.31 & 0.23 & 0.03 & 1.03 \\
% \hline
% & \mollmTripleTaskM & 71.00 & 0.59 & 100.00 & 3.29 & 0.87 & 0.71 & 0.12 & -0.33 & 0.36 & 0.11 & 1.68 \\
% & \mollmTripleTaskL & 77.80 & 0.57 & 100.00 & 3.08 & 0.85 & 0.70 & 0.16 & -0.02 & 0.35 & 0.15 & 2.15 \\
% & \mollmQuadTaskM & 45.00 & 0.63 & 100.00 & 3.25 & 0.86 & 0.61 & 0.08 & -0.68 & 0.26 & 0.07 & 1.53 \\
% & \mollmQuadTaskL & 44.80 & 0.70 & 100.00 & 3.41 & 0.88 & 0.65 & 0.06 & -1.25 & 0.31 & 0.05 & 1.14 \\
% \hline
% & \mollmTripleGenM & 71.00 & 0.60 & 100.00 & 3.22 & 0.87 & 0.67 & 0.13 & -0.16 & 0.32 & 0.12 & 2.09 \\
% & \mollmTripleGenL & 69.40 & 0.58 & 99.71 & 3.16 & 0.87 & 0.72 & 0.12 & -0.21 & 0.37 & 0.11 & 1.96 \\
% & \mollmQuadGenM & 72.80 & 0.61 & 100.00 & 3.26 & 0.87 & 0.67 & 0.13 & -0.18 & 0.33 & 0.12 & 1.94 \\
% & \mollmQuadGenL & 67.60 & 0.58 & 99.70 & 3.13 & 0.87 & 0.69 & 0.12 & 0.06 & 0.35 & 0.11 & 2.17 \\
% \bottomrule
% \end{tabular}



\begin{tablenotes}
\footnotesize
\setlength\labelsep{0pt}
    \item $^\uparrow$ and $^\downarrow$ denote whether a higher or lower value of the metric is desirable, respectively.
    The best-performing {\mollm} is in \textbf{bold} and the best-performing baseline is in \underline{underlined}.  
    % {\SR} represents the success rate, defined as the percentage of cases where the output molecule exhibits better properties than the input molecule.
    % {\Sim} denotes the Tanimoto similarity of the successfully optimized molecule with the input molecule.
    % {\Nov} denotes the percentage of optimized molecules that are not present in the training set.
    % {\SAS} denotes synthetic accessibility score, with lower values indicating easier synthesis.
    %{\Div} represents the diversity or dissimilarity among the optimized molecules.
    %{\Imp} denotes the average improvement across all the involved properties in the task.
\par
\end{tablenotes}

\end{threeparttable}
\end{table*}
